Obtaining Game-Stationary Points for Smooth Nonconvex-Nonconcave Minimax Problems via First-Order Methods

Minimax optimization is a fundamental framework in machine learning, robust optimization, and game theory, yet finding first-order stationary points of general nonconvex-nonconcave minimax problems remains challenging without additional structural assumptions. Existing guarantees often rely on global PL- or KL-type conditions that connect max-player stationarity to global inner optimality, or on Minty-type conditions that impose a global relation on the game gradient field relative to a reference solution; local KL variants relax the former requirement but typically require initialization and tracking within a near-optimal region. Such conditions may be difficult to satisfy in many applications. In contrast, we develop a first-order method that finds an $\epsilon$-stationary point within $\widetilde{O}(\epsilon^{-2})$ first-order iterations under a local inverse-Lipschitz regularity condition around approximate max-player stationary points, together with a compactness condition on a penalty sublevel set. Our condition places no optimality requirement on stationary points of the inner maximization problem: they need not be globally, or even locally, maximizing. We further provide sufficient conditions for the required regularity. In the unconstrained setting, it follows from uniform nonsingularity of the maximization-variable Hessian near stationary points; for constrained upper Moreau envelopes, it follows from standard KKT regularity conditions. These results establish first-order complexity guarantees for classes of nonconvex-nonconcave minimax problems not covered by the above PL-, KL-, or Minty-type frameworks.

==> introduction_v3.tex <==
\section{Introduction}
\label{sec:introduction}
Minimax optimization is a basic modeling framework for machine learning and engineering, including
adversarial training, robust optimization, generative modeling, multi-agent systems,
fair representation learning, reinforcement learning and robust
control
\citep{goodfellow2014gan,madry2018adversarial,sinha2018distributional,
madras2018fair,dai2018sbeed,nachum2019dualdice,basar2008hinfinity, ozdaglar2023revisiting}.

A minimax problem takes the following form:
\begin{equation}
\min_{x\in\mathbb{R}^d}\max_{y\in\mathbb{R}^m} F(x,y).
    \label{eq:intro-minimax}
\end{equation}
Convex--concave instances of \eqref{eq:intro-minimax} admit a mature theory
based on monotone variational inequalities
\citep{nemirovski2004prox,mokhtari2020unified,hamedani2021linesearch,
zhang2024robust,zheng2026lastiterate}.%When only the minimizing side is nonconvex, one can use gradient-descent--ascent-type, two-timescale, or smoothed methods
When only the minimizing component is nonconvex, existing approaches include gradient descent–ascent methods, two-timescale algorithms, and smoothing techniques \citep{lin2020gda,rafique2022weakly,nouiehed2019solving,kong2021accelerated,
zhang2021complexity,zhang2020smoothedgda,yang2022faster}.
However, these methods do not readily extend to the \emph{nonconvex–nonconcave} (NC-NC) regime, where the absence of convexity and concavity presents substantial additional challenges. 
%The \emph{nonconvex--nonconcave} (NC--NC) regime is qualitatively different:
%gradient descent--ascent can cycle or diverge, even the appropriate local solution concept requires care, and the general problem is computationally hard \citep{jin2020localminimax,grimmer2023landscape,daskalakis2021complexity, diakonikolas2021efficient}.
Indeed, several existing works \citep{jin2020localminimax,grimmer2023landscape,daskalakis2021complexity, diakonikolas2021efficient} have highlighted the difficulties inherent in this setting. For instance, gradient descent–ascent methods may exhibit cyclic behavior or diverge, the choice of an appropriate local solution concept requires careful consideration and solving the general nonconvex–nonconcave problem is computationally challenging.

Motivated by these challenges, we study the nonconvex-nonconcave setting and our goal is to find a 
%This paper studies the basic computational goal of finding a
\emph{joint first-order stationary point}, i.e., a
pair $(x,y)$ with
\begin{equation}
    \nabla_x F(x,y)=0,
    \qquad
    \nabla_y F(x,y)=0,
    \label{eq:intro-joint-stationarity}
\end{equation}
and, more precisely, an $\epsilon$-approximate version of \eqref{eq:intro-joint-stationarity} measured by
$\|\nabla_xF(x,y)\|+\|\nabla_yF(x,y)\|\leq\epsilon$. 

% Explain its usefulness
Although joint first-order stationarity is weaker than local or global minimax optimality, it remains a basic computational target for smooth games: it is a necessary condition for every smooth minimax point and the associated residual can be evaluated directly without solving a global inner maximization problem. 

% Review value-function stationarity methods

% Review game/operator stationarity methods

% identify the gap

% introduce our transfer


% Neither direct descent nor descent-ascent is covered by our setting. Standard descent analysis for \(F\) requires a finite objective-decrease gap, whereas \(F\) may be unbounded below in the max-player direction. Descent-ascent is also unsuitable because our framework permits nondegenerate local minima in \(y\). We instead construct a smooth descent penalty whose stationarity transfers to \(F\).

% \paragraph{Prior work and the question addressed.}
% Many guarantees for nonconvex--nonconcave problems rely on additional global structure. 
% For example, a one-sided Polyak--\L{}ojasiewicz or gap-based
% Kurdyka--\L{}ojasiewicz (KL) condition bounds the distance to the max-player's
% \emph{global} value $F^\star(x):=\sup_yF(x,y)$ by a max-player stationarity
% residual; when imposed at every max-player critical point, such a condition
% rules out suboptimal critical points
% \citep{nouiehed2019solving,yang2022faster,zheng2023universal,
% li2025primaldual}. Minty variational inequalities instead posit a globally
% coherent reference solution \citep{diakonikolas2021efficient,pethick2022escaping}.
% The local KL condition of \citet{luwang2026constrainedminimax} is more
% permissive: it is imposed only in a near-optimal region, which can contain no
% suboptimal stationary points, and their method tracks that region from a
% suitable initial inner solution. These methods address different problem
% classes and, in some cases, stronger stationarity notions for the maximal-value
% problem.
Many guarantees for nonconvex--nonconcave problems relate max-player
stationarity to the global value $F^\star(x) := \sup_y F(x,y)$. A one-sided
Polyak--\L{}ojasiewicz (PL) condition \citep{nouiehed2019solving,yang2022faster} requires
$\|\nabla_yF(x,y)\|^2\geq2\mu\bigl(F^\star(x)-F(x,y)\bigr)$;
a global gap-based Kurdyka--\L{}ojasiewicz (KL) condition \citep{zheng2023universal,li2025primaldual} on a feasible set
$\mathcal Y$ imposes an analogous bound
$\operatorname{dist}\bigl(0,-\nabla_yF(x,y)+N_{\mathcal Y}(y)\bigr)
    \geq c\bigl(F^\star(x)-F(x,y)\bigr)^\theta$.
Wherever these inequalities
hold, all stationary point in the region must be globally optimal on the structured side.
A different line assumes a Minty variational inequality (MVI): in the
unconstrained case, some $z^\star$ satisfies
$\langle G(z),z-z^\star\rangle\geq0$ for every $z$, where
$G=(\nabla_xF,-\nabla_yF)$; it implies that $z^\star$ is a global saddle
point and hence a joint stationary point. However, its global reference point
can be difficult to verify and is inapplicable to many nonconvex--nonconcave
objectives \citep{zheng2023universal}. Weak MVI
allows a negative residual, for example
$\langle G(z),z-z^\star\rangle\geq-\eta\|G(z)\|^2$ for an admissible
$\eta>0$; the permitted range has been enlarged by subsequent methods, but
the condition still relates every $z$ to one reference solution
\citep{diakonikolas2021efficient,pethick2022escaping,fan2024weaker}.

Very recently, \citet{luwang2026constrainedminimax} substantially
relax global KL: they require the KL inequality only on an $x$-dependent
near-optimal level set, which allows suboptimal stationary points outside that
region. Their algorithmic guarantee, however, relies on starting in and subsequently tracking this near-global region: the initial inner point must be a
suitable approximate solution of the first maximization problem, and obtaining such a point with their inner solver requires an initialization in a region where the
local KL condition already holds, unless the first inner problem has
additional favorable structure; each subsequent inner problem is then
initialized from the preceding inner solution.

This motivates our question:
\begin{center}
\emph{Can we find a joint stationary point without requiring max-player stationarity to certify global optimality or assuming globally coherent solutions or initializing near the global maximizer set?}
\end{center}
We answer affirmatively. Under a compact penalty sublevel set and a local
condition at the max-player critical points inside it, a single smooth penalty
transfers its own approximate stationarity to $F$, and gradient descent on
that penalty reaches an $\epsilon$-joint-stationary point within
$\widetilde{O}(\epsilon^{-2})$ total gradient evaluations.

\paragraph{Our reformulation.}
Suppose that $F$ is $L$-smooth, and fix $p>L$. Define
the regularized best response and its gap
\begin{equation}
    w(x,y)
    :=\arg\max_{v\in\mathbb{R}^m}
    \left\{F(x,v)-\frac{p}{2}\|v-y\|^2\right\},
    \label{eq:w-def}
\end{equation}
\begin{equation}
    \mathcal{G}(x,y)
    :=F(x,w(x,y))-
      \frac{p}{2}\|w(x,y)-y\|^2-F(x,y).
    \label{eq:G-def}
\end{equation}
The inner problem in \eqref{eq:w-def} is $(p-L)$-strongly concave even when
$F(x,\cdot)$ is nonconcave. Consequently, $w$ is single-valued,
$\mathcal{G}\geq0$, and $\mathcal{G}(x,y)=0$ exactly when
$\nabla_yF(x,y)=0$ (Lemma~\ref{lem:gap-properties}). Penalizing this gap gives
the smooth objective
\begin{equation}
    P_\rho(x,y):=F(x,y)+\rho\mathcal{G}(x,y),\qquad \rho>0.
    \label{eq:Prho-def}
\end{equation}
By Danskin's theorem, $\nabla P_\rho(x,y)$ is computed from first-order
information at $(x,y)$ and $(x,w(x,y))$ alone, so minimizing $P_\rho$ is an
ordinary smooth nonconvex minimization problem.

\paragraph{Stationary exactness at a finite penalty parameter.}
Smooth merit functions for nonconvex games have been proposed before
\citep{raghunathan2019gni,tsaknakis2021fne}. In those settings the
\emph{global minimizers} of the merit function encode joint stationarity. However, the
merit function is itself nonconvex, so a first-order method returns
only a \emph{stationary point} of it, and a stationary point alone does not in
general certify joint stationarity of the original problem. Our analysis
closes this gap under a local condition: a finite $\bar\rho$, independent of
the target accuracy, can be chosen so that for every fixed $\rho\ge\bar\rho$,
\begin{equation}
    P_\rho(x,y)\leq C_0,\quad
    \|\nabla P_\rho(x,y)\|\leq\varepsilon
    \quad\Longrightarrow\quad
    \|\nabla_xF(x,y)\|+\|\nabla_yF(x,y)\|
    \leq C_\rho\varepsilon,
    \label{eq:intro-transfer}
\end{equation}
with an explicit constant $C_\rho$ (Theorem~\ref{thm:stationarity-transfer}).
At $\varepsilon=0$, every stationary point of the penalty in the sublevel set
is a joint stationary point of $F$
(Corollary~\ref{cor:stationary-exactness}).

Under our smoothness assumptions, $P_\rho$ is smooth with a Lipschitz gradient,
\eqref{eq:intro-transfer} converts the standard complexity of smooth nonconvex
minimization into a guarantee for the original problem. Gradient descent on
$P_\rho$ needs $O(\epsilon^{-2})$ outer iterations
(Theorem~\ref{thm:gd-complexity}), and since the best-response problem
\eqref{eq:w-def} is strongly concave and can be solved to the required
accuracy in $O(\log(1/\epsilon))$ ascent steps, the total cost is
$\widetilde{O}(\epsilon^{-2})$ gradient evaluations of $F$
(Theorem~\ref{thm:inexact-gd-complexity}). This is the canonical rate of
gradient descent for finding an $\epsilon$-stationary point of a smooth
nonconvex function, now obtained for joint stationarity of a
nonconvex--nonconcave minimax problem.

\paragraph{The regularity condition.} Let
$\mathcal{K}:=\{(x,y):P_{\rho_c}(x,y)\leq C_0\}$ be a compact sublevel set,
and suppose an initial point with $P_\rho\leq C_0$ is available for each
penalty parameter considered (Assumption~\ref{ass:compact-sublevel}). Our
local condition says that, uniformly for
$(x,y)\in\mathcal{K}$ with both $\|\nabla_yF(x,y)\|$ and
$\|w(x,y)-y\|$ sufficiently small,
\begin{equation}
    \|w(x,y)-y\|
    \leq\kappa_s\|
       \nabla_yF(x,w(x,y))-\nabla_yF(x,y)\|.
    \label{eq:intro-secant-condition}
\end{equation}
This restricted inverse-Lipschitz condition (Assumption~\ref{ass:inverseLip})
only compares the proximal pair $y,w(x,y)$; it makes no reference to
$F^\star(x)$. For $C^2$ objectives, nonsingularity of the max-player Hessian
at critical points in $\mathcal K$ suffices, regardless of the signs of its
eigenvalues (Proposition~\ref{prop:hessian-nondegeneracy}). Thus the condition
permits both local maxima and suboptimal local minima on the max-player side.
For upper Moreau envelopes with a strongly convex constraint, strict
complementarity and nonsingularity of the reduced Lagrangian Hessian provide
another sufficient condition
(Proposition~\ref{prop:constrained-envelope-inverseLip}).

% \paragraph{Organization.}
% Section~\ref{sec:regularized-gap-penalty} develops the regularized gap
% penalty, states the assumptions, and establishes the two sufficient conditions
% for \eqref{eq:intro-secant-condition}.
% Section~\ref{sec:transfer-and-complexity} proves the stationarity transfer
% \eqref{eq:intro-transfer} and the resulting complexity guarantees for gradient
% descent on $P_\rho$ with exact and with inexact best responses. Omitted proofs
% are deferred to the appendix.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

